Multi-focal Conditioned Latent Diffusion for Person Image Synthesis

The Latent Diffusion Model (LDM) has demonstrated strong capabilities in high-resolution image generation and has been widely employed for Pose-Guided Person Image Synthesis (PGPIS), yielding promising results. However, the compression process of LDM often results in the deterioration of details, particularly in sensitive areas such as facial features and clothing textures. In this paper, we propose a Multi-focal Conditioned Latent Diffusion (MCLD) method to address these limitations by conditioning the model on disentangled, pose-invariant features from these sensitive regions. Our approach utilizes a multi-focal condition aggregation module, which effectively integrates facial identity and texture-specific information, enhancing the model's ability to produce appearance realistic and identity-consistent images. Our method demonstrates consistent identity and appearance generation on the DeepFashion dataset and enables flexible person image editing due to its generation consistency. The code is available at https://github.com/jqliu09/mcld.

==> sec/2_related.tex <==
\section{Related Works}
\label{sec:related}


\noindent\textbf{Pose-Guided Person Image Synthesis} aims to translate a source person image with a pose into a given new pose while preserving the appearance of the source person. Generative techniques, including Generative Adversarial Networks~\cite{goodfellow2014generative} and Diffusion Models~\cite{ho2020denoising}, have been widely employed in this task, achieving significant advancements in maintaining appearance consistency and pose accuracy. 

Pose-transfer task was initially proposed by PG2~\cite{ma2017pose} which firstly applies conditional GANs to pose-guided person generation. The main contributions line in two stages learning with an U-Net to learn the image mapping. However, the photorealistic person generation with accurate preservation of complex textures is beyond the reach of this model, as it cannot handle large spatial variations and non-rigid deformation between different poses. Other studies mainly explored ways to handle the deformation between different poses, including using affine transformations~\cite{siarohin2018deformable,siarohin2021PAMI}, spatial (cross) attention~\cite{zhu2019progressive,zhou2021cocosnet,tang2020bipartite,zhang2021pise,men2020controllable,ren2022neural}, flow field~\cite{ren2020deep,ren2021flow,ren2021combining,li2019dense}. For example, flow fields can be estimated by both source and target keypoints, then, CFLA~\cite{ren2020deep} utilizes learned flow fields to warped the features from source appearance into the target-pose space. 

Due to the instability in training and the mode collapse issues associated with GAN models, previous works based on GANs have encountered challenges with unrealistic textures in posed person images. PIDM was the first to utilize the original diffusion model in this generation task, replacing GANs. To blend the texture of the source image into the target pose, PIDM introduces Texture Diffusion Blocks with cross-attention into the denoising U-Net. Subsequent methods~\cite{han2023controllable,lu2024coarse} have sought to improve inference speed by employing diffusion models in latent space rather than pixel space, inspired by Stable Diffusion. For example, CFLD~\cite{lu2024coarse} addresses the limitations of existing approaches that align appearance with target poses, which often suffer from overfitting due to a lack of semantic understanding. To mitigate this, CFLD utilizes a perception-refined decoder to extract coarse-grained semantic prompts and decouple fine-grained appearance and pose controls. Additionally, a hybrid-granularity attention module enhances texture realism through multi-scale feature encoding. \jichao{However, these latent diffusion-based methods struggle to accurately recover the details of the source human images' appearance, particularly in the facial and clothing regions. Thus, this paper introduces a multi-focal conditional method that leverages human faces and texture maps as additional conditions to preserve the appearance of both the face and clothing.}

In addition to utilizing skeletons or keypoints as pose representations in most baseline methods, some approaches~\cite{grigorev2019coordinate,zablotskaia2019dwnet,sarkar2020neural,han2023controllable} leverage DensePose (UV coordinates) to guide person generation, as it provides much denser structural pose and shape information compared to traditional body skeletons. Furthermore, prior works~\cite{Sarkar2021HumanGANAG,sarkar2020neural,grigorev2019coordinate,li2019dense} have explored the integration of 3D information into this task. For instance, HumanGAN~\cite{Sarkar2021HumanGANAG} employs 3D UV texture maps to represent person images and DensePose for keypoint representation, capitalizing on the advantages of pose invariance and shape invariance inherent in texture mapping to reduce the complexity associated with pose transformations. In this paper, we also utilize UV maps as an additional representation and employ DensePose for pose control.

Similar to this task, several advanced video generation methods have been proposed~\cite{siarohin2019first,liu2021liquid,liu2019liquid,siarohin2021motion,ren2021flow,karras2023dreampose,hu2024animate}, which focus on transferring poses from source videos to target videos. However, we do not consider these models as baselines for our work, as our approach does not necessitate video sequences as training data.

\noindent\textbf{Diffusion Models.}
Diffusion models, such as Denoising Diffusion Probabilistic Models (DDPM)~\cite{ho2020denoising}, are generative models that transform noise from a simple distribution into samples from a learned data distribution through an iterative denoising process. To mitigate the extensive number of iterations typically required to produce an image in DDPM, Denoising Diffusion Implicit Models (DDIM)~\cite{pmlr-v202-song23k} employ non-Markovian diffusion processes that can be simulated in fewer steps. Both DDPM and DDIM have established themselves as standards in the realm of diffusion models. Recently, diffusion models have outperformed GANs and significantly improved the visual fidelity of synthesized images across various domains, including text-to-image generation~\cite{rombach2022high,saharia2022photorealistic,ruiz2023dreambooth}, person image generation~\cite{bhunia2023person,lu2024coarse,han2023controllable,xue2024self,cheong2023upgpt}, and 3D avatar generation~\cite{kolotouros2023dreamhuman,cao2023dreamavatar,liao2023tada,huang2023humannorm,poole2022dreamfusion,liu2023zero1to3}. For most tasks, the widely used model is Stable Diffusion~\cite{rombach2022high} (and its variants), which is a unified conditional diffusion model that allows for semantic maps, text, or images to be used as conditions for controlling generation. Its key contributions lie in applying the diffusion process in feature space, which minimizes resource consumption while maintaining generation quality and flexibility. In this paper, our architecture, along with the baseline’s, is derived from Stable Diffusion.


